Grey-Box Learning of Register Automata

Model learning (a.k.a. active automata learning) is a highly effective technique for obtaining black-box finite state models of software components. Thus far, generalisation to infinite state systems with inputs/outputs that carry data parameters has been challenging. Existing model learning tools for infinite state systems face scalability problems and can only be applied to restricted classes of systems (register automata with equality/inequality). In this article, we show how we can boost the performance of model learning techniques by extracting the constraints on input and output parameters from a run, and making this grey-box information available to the learner. More specifically, we provide new implementations of the tree oracle and equivalence oracle from RALib, which use the derived constraints. We extract the constraints from runs of Python programs using an existing tainting library for Python, and compare our grey-box version of RALib with the existing black-box version on several benchmarks, including some data structures from Python's standard library. Our proof-of-principle implementation results in almost two orders of magnitude improvement in terms of numbers of inputs sent to the software system. Our approach, which can be generalised to richer model classes, also enables RALib to learn models that are out of reach of black-box techniques, such as combination locks.

==> figures/SDTs/nonMinimalSDTResult.tex <==
\begin{tikzpicture}[scale=0.8]

\node[state, accepting] (rejecting1) at (0,0) {$-$};
\node[state, accepting] (rejecting2) at (4,0) {$-$};
\node[state, accepting] (accepting1) at (2,0) {$+$};
\node[state, accepting] (accepting2) at (6,0) {$+$};


\node[state, accepting] (s1_neq_r0) at (1,2) {$s_{20}$};
\node[state, accepting] (s1_eq_r0) at (5,2) {$s_{21}$};
\node[state, accepting] (root) at (3,4) {$s_1$};

\path[-Latex] (root) edge [] node[left] {\(s_1 \neq d_0\)} (s1_neq_r0); 
\path[-Latex] (root) edge [] node[right] {\(s_1 = d_0\)} (s1_eq_r0); 

\path[-Latex] (s1_neq_r0) edge [] node[left] {\(s_2 \neq d_0\)} (rejecting1);
\path[-Latex] (s1_eq_r0) edge [] node[left] {\(s_2 \neq s_1\)} (rejecting2);


\path[-Latex] (s1_eq_r0) edge [] node[right] {\(s_2 = s_1\)} (accepting2);
\path[-Latex] (s1_neq_r0) edge [] node[right] {\(s_2 = d_0\)} (accepting1);
  
\end{tikzpicture}
  
  
%%% Local Variables:
%%% TeX-master: "../../document.tex"
%%% End:

==> figures/combinedTex.tex <==
\begin{table}
\centering
\caption{Benchmarks (where T: Tainted, N: Normal). All values are averages.}
\label{tbl:benchmarks}
\begin{small}
%\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|cc|c|rr|rr|r|r}
\toprule
\textbf{Model} & \multicolumn{2}{c|}{\textbf{Oracle}} & \textbf{Rounds} & \multicolumn{2}{c}{\textbf{Learn}} & \multicolumn{2}{|c|}{\textbf{Test}} &   \textbf{Total} &  \textbf{Learned} \\
      &    Tree    &  Equiv.  &        &   Inputs           &    Resets &  Inputs           &   Resets & &       \\
      &            &          &        &  \multicolumn{5}{c|}{~~(in thousands)}  &        \\
  \toprule
  %% SIP-2015 model
SIP &    T &  T &    9.0 &      3.6 &      0.82 &     17 &     0.6 & 22 &   9/11 \\
    &    T &   N &    9.6 &      3.5 &      0.89 &     4.1 &     0.47 & 8.9 &   9/10 \\
  \cmidrule{2-10}
     &     N &  T &    9.0 &      1100 &      120 &     17 &     0.6 & 1300 &    9/09 \\
     &     N &   N &    9.3 &      23 &      3.7 &     4.8 &     0.54 & 32 &  10/10 \\
\midrule
Repetition &    T &  T &    6.0 &      0.075 &      0.047 &     3.5 &     0.19 & 3.9 &  10/10 \\
     &    T &   N &    4.4 &      0.054 &      0.035 &     40 &     4.6 & 45 &   0/10 \\
  \cmidrule{2-10}
     &     N &  T &    6.0 &      5.9 &      3 &     3.5 &     0.19 & 13 &  10/10 \\
     &     N &   N &    4.4 &      4.8 &      2.5 &     4.0 &     4.6 & 52 &   0/10 \\
\midrule
Lock &    T &  T &    2.0 &      0.063 &      0.029 &     0.45 &     0.016 & 0.56 &  10/10 \\
2-digit &     N &  T &    2.0 &      0.14 &      0.056 &     0.45 &     0.016 & 0.66 &  10/10 \\
\midrule
Lock &    T &  T &    2.0 &      0.42 &      0.11 &     4.6 &     0.16 & 5.3 &  10/10 \\
4-digit    &     N &  T &    2.0 &      29 &      5.5 &     4.6 &     0.16 & 39 &  10/10 \\
\midrule
Set-4 &    T &  T &    4.1 &      62 &      6.7 &     1.2 &     0.045 & 70 &  10/10 \\
%%% Not performed     &    T &   N &    nan &          nan &          nan &         nan &         nan &     nan &    0/1 \\
     &     N &  T &    4.0 &      20000 &      1700 &     1.2 &     0.045 & 22000 &   9/10 \\
\midrule
Fifo-5 &    T &  T &    6.6 &      2.6 &      0.45 &     0.24 &     0.021 & 3.3 &  10/10 \\
     &    T &   N &    6.9 &      2.5 &      0.44 &     0.69 &     0.088 & 3.8 &  10/10 \\
  \cmidrule{2-10}
     &     N &  T &    6.6 &      110 &      9.5 &     0.24 &     0.021 & 120 &  10/10 \\
     &     N &   N &    6.9 &      39 &      4 &     0.69 &     0.088 & 44 &  10/10 \\
\midrule
ABP- &    T &  T &    6.6 &      1 &      0.24 &     8.6 &     0.3 & 10 &  10/10 \\
Output     &    T &   N &    7.4 &      1 &      0.24 &     3.5 &     0.38 & 5.1 &   9/10 \\
  \cmidrule{2-10}
     &     N &  T &    6.6 &      230 &      26 &     8.6 &     0.3 & 260 &  10/10 \\
     &     N &   N &    7.4 &      6.6 &      1.4 &     3.5 &     0.38 & 12 &   9/10 \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\end{small}
\end{table}

%%% Local Variables:
%%% TeX-master: "../document.tex"
%%% End:
% LocalWords:  Fifo


==> figures/well_formed/non-well_formed.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
\node[state, accepting,inner sep=1pt,minimum size=15pt] (q_0) {$l_0$}; 
\node[state, accepting,inner sep=1pt,minimum size=15pt] (q_1) at (-1,-2) {};
\node[state,inner sep=1pt,minimum size=15pt] (q_2) at (1,-2) {};
\node[state,inner sep=1pt,minimum size=15pt] (q_3) at (1,-4) {};
\node[state, accepting,inner sep=1pt,minimum size=15pt] (q_4) at (-1,-4) {};

\path[->] (q_0) edge[left] node[align=center] {$\alpha(s_1)$ \\ $s_1 = s_2$} (q_1); 
\path[->] (q_0) edge[right] node[align=center] {$\alpha(s_1)$ \\ $s_1 \ne s_2$} (q_2); 
\path[->] (q_1) edge[left] node[align=center] {$\alpha(s_2)$} (q_4); 
\path[->] (q_2) edge[right] node[align=center] {$\alpha(s_2)$} (q_3); 

\end{tikzpicture}

==> figures/well_formed/well_formed.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
\node[state, accepting,inner sep=1pt,minimum size=15pt] (q_0) {$l'_0$}; 
\node[state, accepting,inner sep=1pt,minimum size=15pt] (q_1) at (0,-2) {};
\node[state,inner sep=1pt,minimum size=15pt] (q_3) at (1,-4) {};
\node[state, accepting,inner sep=1pt,minimum size=15pt] (q_4) at (-1,-4) {};

\path[->] (q_0) edge[left] node[align=center] {$\alpha(s_1)$} (q_1); 
\path[->] (q_1) edge[left] node[align=center] {$\alpha(s_2)$  \\ $s_2 = s_1$} (q_4); 
\path[->] (q_1) edge[right] node[align=center] {$\alpha(s_2)$  \\ $s_2 \ne s_1$} (q_3); 

\end{tikzpicture}

==> sections/relatedWork.tex <==
\section{Related Work}\label{sec:relatedWork}
This section is divided into two portions: the first introduces the early work
of automata learning and efforts towards learning more expressive models, and
the second discusses integration of white-box techniques in automata learning.

Beginning with Angluin's seminal paper~\cite{DanaAngluinBasePaper}, which
introduced the MAT framework and \(L^*\), the first active learning algorithm for deterministic finite
automata, there has been steady progress towards \((a)\) improving the
scalability of active learning and \((b)\) learning richer (i.e., more
expressive) models.
\citet{mealyLearning1, mealyLearning2} extended active learning to inferring
mealy machines, allowing learning of explicit input/output behaviour.
Additionally, the TTT algorithm~\cite{tttAlgorithm} improved scalability of
counterexample analysis as compared to the \(L^*\) algorithm.
Improvements in equivalence testing for mealy machines have also played a role
in improving scalability of the same~\cite{wMethod, wpMethod,
  improveTestingMethod}.
Learning of models with \emph{infinite} statespaces as register automata was
proposed by~\cite{10.1007/978-3-642-27940-9_17}.
Data parameters could be stored in registers with equality guards being defined
over those parameters.
Register automata were then extended to support richer operations as
well and could be used to learn models of data structures, amongst
others~\cite{raLibFirstPaper,cassel2015ralib,Cassel2016}.
However, these black-box approaches lead to scalability issues.

In order to improve scalability, there has been some work done in integrating
white-box techniques in automata learning: the authors
of~\cite{symbolicComponentInterfaces, sigmaStar, mace}
all use some form of symbolic or `concolic' (concrete + symbolic) execution in
order to improve scalability of active automata learning.
In this work, we use tainting to reduce the number of inputs needed to learn a
model with guards based on equality operations between data parameters.
We use `tainting' in a distinct sense from the commonly-used technique for
security analysis~\cite{Schwartz2010a}, which is --- at risk of
over-simplification --- an information flow technique.
In the context of this work, `tainting' indicates knowledge of what is
`happening' to a data variable, and not the flow of the variable through a
program.


%%% Local Variables:
%%% TeX-master: "../document.tex"
%%% reftex-default-bibliography: ("../reference.bib")
%%% End:

